FusionPortableV2: A Unified Multi-Sensor Dataset for Generalized SLAM Across Diverse Platforms and Scalable Environments

Simultaneous Localization and Mapping (SLAM) technology has been widely applied in various robotic scenarios, from rescue operations to autonomous driving. However, the generalization of SLAM algorithms remains a significant challenge, as current datasets often lack scalability in terms of platforms and environments. To address this limitation, we present FusionPortableV2, a multi-sensor SLAM dataset featuring sensor diversity, varied motion patterns, and a wide range of environmental scenarios. Our dataset comprises $27$ sequences, spanning over $2.5$ hours and collected from four distinct platforms: a handheld suite, a legged robots, a unmanned ground vehicle (UGV), and a vehicle. These sequences cover diverse settings, including buildings, campuses, and urban areas, with a total length of $38.7km$. Additionally, the dataset includes ground-truth (GT) trajectories and RGB point cloud maps covering approximately $0.3km^2$. To validate the utility of our dataset in advancing SLAM research, we assess several state-of-the-art (SOTA) SLAM algorithms. Furthermore, we demonstrate the dataset's broad application beyond traditional SLAM tasks by investigating its potential for monocular depth estimation. The complete dataset, including sensor data, GT, and calibration details, is accessible at https://fusionportable.github.io/dataset/fusionportable_v2.

==> chapter/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Potential Extensions}

This paper mainly focuses on the localization and mapping tasks, where detailed ground truth and complete evaluation are presented. 
The key feature of our proposed dataset is that the uniform multi-sensor setting, multiple type of robots with onboard sensor data, and various scenarios (\textit{e.g.,} building, street, highway). 
The proposed dataset provides multiple types of sensor measurements, various scenarios, and robot platforms at diverse motion features. 
Based on the fundamental localization and mapping tasks, we believe that the proposed dataset can boost the development and evaluation of many tasks regarding other tasks for robotics. 
We provide several possible extensions:
\begin{itemize}[leftmargin=0.35cm]
    \item \textbf{SLAM with the Combination of Geometric and End-to-End Methods}: xxx
    \item \textbf{Perception}: object detection, segmentation, prediction, depth estimation.
    \item \textbf{NeRF-based Mapping}: 
    The recent progress of NeRF is amazing, which has evolved existing frameworks in 3D reconstruction and AR/VR. There still exist many research opportunies and unsolved problems in robotics, such as mapping the large-scale field environments (unboundaried environments), multi-sensor fusion-based NeRF (including LiDARs, cameras, event cameras), NeRF-based place recognition, and NeRF-based navigation. Our dataset provides valuable data for researching this field, and several researchers have made some trials \citep{}.
    \item \textbf{Navigation for General Mobile Robots}:
    path planning, interaction, imitation learning, supervised and unsupervised learning.
\end{itemize}

\bt{TODO by jjiao: provide a figure to overview the potential applications of the proposed dataset}

==> figure/fig_device_timing.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=0.44\textwidth]{image/layout/device_timing-crop.pdf}
    \caption{Timing diagram of triggerable and non-triggerable sensors, illustrating their synchronization and timestamping processes. }
    \label{fig:device_timing}
    \vspace{-0.4cm}
\end{figure}

==> figure/fig_point_cloud_station.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \subfigure[Campus]{
            \label{fig:gt_map_quality_campus}
            \includegraphics[width=0.45\linewidth]{./image/experiment/station-crop.pdf}
        }
        \subfigure[Underground tunnel]{
            \label{fig:gt_map_quality_tunnel}
            \includegraphics[width=0.45\linewidth]{./image/experiment/underground_scan_crop.pdf}
        }
    \end{minipage}
    \caption{Position of all stations of underground scenarios.}
    \label{fig:rgb_point_cloud_station}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

